Identification of an X-ray Pulsar in the BeXRB system IGR J18219$-$1347

We report on observations of the candidate Be/X-ray binary IGR J18219$-$1347 with \textit{Swift}/XRT, \textit{NuSTAR}, and \textit{NICER} during Type-I outbursts in March and June 2020. Our timing analysis revealed the spin period of a neutron star with $P_\textrm{spin}=52.46$ s. This periodicity, combined with the known orbital period of $72.4$ d, indicates that the system is a BeXRB. Furthermore, by comparing the infrared counterpart's spectral energy distribution to known BeXRBs, we confirm this classification and set a distance of approximately $10-15$ kpc for the source. The source's broadband X-ray spectrum ($1.5-50$ keV) is described by an absorbed power-law with photon index $\Gamma$\,$\sim$\,$0.5$ and cutoff energy at $\sim$\,$13$ keV.

==> old_tables.tex <==
\begin{table}
    \centering
    \caption{Spectral parameters from a combined \textit{NuSTAR} and \textit{NICER} fit (time-averaged) in the $1.5-50$ keV energy range. \brendan{only the cutoffpl model provides a decent description (see Figure \ref{fig: joint_nicer+nustar_fit}). the other two in this table are absolutely awful fits! I think we should only report the cutoffpl component for all fits... can we ignore the bb description of NICER??
    }
    }
    \label{tab: nustar+nicer}
    \begin{tabular}{lccc}
    \hline
    \hline
   \textbf{Parameter}  & \textbf{Value} & \textbf{Units}  \\
    \hline
    \hline
    \multicolumn{3}{c}{\textbf{Model 1: \texttt{tbabs*pow}}} \\
     \hline
     \hline
      $N_H$   &  & $10^{22}$ cm$^{-2}$ \\
      $\Gamma$  &  &  \\
       $F_X$($2-50$ keV)  & & $10^{-10}$ erg cm$^{-2}$ s$^{-1}$   \\
      Cstat &  & \\
    \hline
    \hline
    \multicolumn{3}{c}{\textbf{Model 2: \texttt{tbabs*cutoffpl}}} \\
     \hline
     \hline
           $N_H$   & $8.3\pm0.3$  & $10^{22}$ cm$^{-2}$ \\
      $\Gamma$  & $0.51\pm0.03$ &  \\
    $E_\textrm{cut}$   & $13.3\pm0.04$ & keV  \\
       $F_X$($2-50$ keV)  & $1.37\pm0.02$ & $10^{-10}$ erg cm$^{-2}$ s$^{-1}$   \\
      Cstat & 2130 (1929 d.o.f)  & \\
     \hline
     \hline
        \multicolumn{3}{c}{\textbf{Model 3: \texttt{tbabs*(pow+bb)}}} \\
     \hline
     \hline
           $N_H$   &  & $10^{22}$ cm$^{-2}$ \\
      $\Gamma$  &  &  \\
      kT & & keV \\
       $F_X$($2-50$ keV)  & & $10^{-10}$ erg cm$^{-2}$ s$^{-1}$   \\
      Cstat &  & \\
     \hline
     \hline
    \end{tabular}
\end{table}



\begin{table}
    \centering
    \caption{Best fit spectral parameters from \textit{NICER} (time-averaged) in the $1.5-12$ keV range. Confidence intervals are at the 68\% level.
    }
    \label{tab: spectral fit nicer}
    \begin{tabular}{lccc}
    \hline
    \hline
     \textbf{Parameter}  & \textbf{Value} & \textbf{Units}  \\
    \hline
    \hline
        \multicolumn{3}{c}{\textbf{Model 1: \texttt{tbabs*pow}}} \\
            \hline
    \hline
      $N_H$   & $8.09\pm0.37$ & $10^{22}$ cm$^{-2}$ \\
      $\Gamma$  & $0.81\pm0.07$ &  \\
       $F_X$($2-10$ keV)  & $6.92\pm0.12$ & $10^{-11}$ erg cm$^{-2}$ s$^{-1}$   \\
   Cstat & 745 (685 d.o.f) & \\
    \hline
    \hline
    \multicolumn{3}{c}{\textbf{Model 2: \texttt{tbabs*cutoffpl}}} \\
     \hline
     \hline
           $N_H$   & $7.4\pm0.4$  & $10^{22}$ cm$^{-2}$ \\
      $\Gamma$  & $0.37\pm0.07$ &  \\
    $E_\textrm{cut}$   & $14$ (frozen) & keV  \\
       $F_X$($2-10$ keV)  & $6.69\pm0.12$ & $10^{-11}$ erg cm$^{-2}$ s$^{-1}$   \\
      Cstat & 734 (685 d.o.f)  & \\
  %   \hline
  %   \hline
  %      \multicolumn{3}{c}{\textbf{Model 3: \texttt{tbabs*(pow+bb)}}} \\
   %  \hline
   %  \hline
   %        $N_H$   & $5.3^{+0.5}_{-0.4}$  & $10^{22}$ cm$^{-2}$ \\
    %  $\Gamma$  & $3.8^{+5.6}_{-1.8}$ &  \\
    %  kT & $2.23\pm0.07$ & keV \\
    %   $F_X$($2-10$ keV)  & $5.97\pm0.15$ & $10^{-11}$ erg cm$^{-2}$ s$^{-1}$   \\
   %   Cstat & 745 (721 d.o.f) & \\
         \hline
     \hline
        \multicolumn{3}{c}{\textbf{Model 3: \texttt{tbabs*bb}}} \\
     \hline
     \hline
           $N_H$   & $5.0\pm0.3$  & $10^{22}$ cm$^{-2}$ \\
      kT & $2.25\pm0.07$ & keV \\
       $F_X$($2-10$ keV)  & $5.91\pm0.13$ & $10^{-11}$ erg cm$^{-2}$ s$^{-1}$   \\
      Cstat & 711 (685 d.o.f) & \\
     \hline
     \hline
    \end{tabular}
\end{table}


\begin{table}
    \vspace{5mm}
    \centering
    \caption{Best fit (time-averaged) spectral parameters from \textit{NuSTAR} using \texttt{XSPEC} in the $3-50$ keV range. 
    }
    \label{tab: spectral fit}
    \begin{tabular}{lccc}
    \hline
    \hline
    \textbf{Parameter}  & \textbf{Value} & \textbf{Units}  \\
   % \hline
   % \hline
   %     \multicolumn{3}{c}{\textbf{Model 1: \texttt{tbabs*pow}}} \\
   %         \hline
   % \hline
   %   $N_H$   & bad fit & $10^{22}$ cm$^{-2}$ \\
   %   $\Gamma$  &  &  \\
   %    $F_X$($2-10$ keV)  &  & $10^{-10}$ erg cm$^{-2}$ s$^{-1}$   \\
  % Cstat & 2154 (1246 d.o.f) & \\
   % \hline
   % \hline
    \multicolumn{3}{c}{\textbf{Model: \texttt{tbabs*cutoffpl}}} \\
     \hline
     \hline
      $N_H$   & $11.24\pm0.74$ & $10^{22}$ cm$^{-2}$ \\
      $\Gamma$  & $0.65\pm0.04$ &  \\
      $E_\textrm{cut}$   & $14.7\pm0.6$ & keV  \\
%       $A$  & $4.13^{+0.05}_{-0.04}$ & $10^{-3}$  \\
    %     & &  \\
       $F_X$($3-50$ keV)  & $1.93\pm0.02$ & $10^{-10}$ erg cm$^{-2}$ s$^{-1}$   \\
       Cstat & 1377 (1245 d.o.f) & \\
     \hline
     \hline
    \end{tabular}
\end{table}

